Squeeze Out Tokens from Sample for Finer-Grained Data Governance

Widely observed data scaling laws, in which error falls off as a power of the training size, demonstrate the diminishing returns of unselective data expansion. Hence, data governance is proposed to downsize datasets through pruning non-informative samples. Yet, isolating the impact of a specific sample on overall model performance is challenging, due to the vast computation required for tryout all sample combinations. Current data governors circumvent this complexity by estimating sample contributions through heuristic-derived scalar scores, thereby discarding low-value ones. Despite thorough sample sieving, retained samples contain substantial undesired tokens intrinsically, underscoring the potential for further compression and purification. In this work, we upgrade data governance from a 'sieving' approach to a 'juicing' one. Instead of scanning for least-flawed samples, our dual-branch DataJuicer applies finer-grained intra-sample governance. It squeezes out informative tokens and boosts image-text alignments. Specifically, the vision branch retains salient image patches and extracts relevant object classes, while the text branch incorporates these classes to enhance captions. Consequently, DataJuicer yields more refined datasets through finer-grained governance. Extensive experiments across datasets demonstrate that DataJuicer significantly outperforms existing DataSieve in image-text retrieval, classification, and dense visual reasoning.

==> content/fig/scaling/modelscaling/fig.tex <==
\begin{figure}[htpb]
% \begin{wrapfigure}[10]{r}{0.21\textwidth}

\centering
\begin{subfigure}{0.20\textwidth}
    \centering
    % \includegraphics[width=\textwidth]{content/fig/scaling/modelscaling/modelscale.png}
    \includegraphics[width=\textwidth]{content/fig/scaling/modelscaling/modelscale.pdf}
    % \caption{Loss.}
    \label{fig:first}
\end{subfigure}
% \hfill

% \vspace{-15pt}
% \caption{\textbf{Model Scaling.} Performance of TinyLlama pre-trained under our DiSF with 1.5\% selection budget compared}

\label{fig:modelscaling}

% \end{wrapfigure}
\end{figure}


==> content/tab/ablation/infer.tex <==

\begin{table}[t]
    \centering
    \footnotesize
    \caption{\textbf{Ablation of Inference-time Image Condensation}. VLMs trained with half patches dropped are compatible with different number of patches during inference.}
    % \vspace{-0.3cm}
    \begin{tabular}{lc|cc|cc}
        \toprule
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Speed-Up} & \multicolumn{2}{c|}{MSCOCO} & \multicolumn{2}{c}{Flickr} \\
        ~ & ~ & I2T & T2I & I2T & T2I \\
        \hline \hline
        FullPatch  0\% & 0 & 26.9 & 28.1 & 47.7 & 47.7 \\
        \midrule
        RandDrop 50\% & 22 & 26.5 & 28.2 & 47.2 & 46.8 \\
        RandDrop 75\% & 31 & 24.3 & 26.6 & 44.0 & 44.2 \\
        \midrule
        GuideDrop 50\% & 22 & 27.4 & 29.1 & 48.2 & 47.8 \\
        GuideDrop 75\% & 31 & 25.6 & 27.6 & 46.3 & 46.2 \\
        \bottomrule
    \end{tabular}
    \label{tab:infer}
\end{table}




==> content/tab/ablation/patch.tex <==

\begin{table}[t]
    \centering
    \footnotesize
    \caption{\textbf{Ablation of Image Condensation}. The dropping rate of image patches indicates the degree of condensation. We demonstrate downstream tasks requiring different semantic granularity determine the choice of input patch numbers.}
    % \vspace{-0.3cm}
    \begin{tabular}{l|cccc|cc}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{2}{c}{MSCOCO} & \multicolumn{2}{c|}{ImgNet} & \multirow{2}{*}{OKVQA} & \multirow{2}{*}{HalBench} \\
        ~ & I2T & T2I & Top1 & Top5 \\
        \hline \hline
        Rand & 23.1 & 23.4 & 10.08 & 22.68 & 34.24 & 29.12 \\
        \midrule
        BTS & 26.5 & 27.8 & 10.56 & 23.27 & 50.48 & 27.76 \\
        \midrule
        Ours 25\% & 22.9 & 23.1 & 12.47 & 32.11 & 42.18 & 27.21 \\
        Ours 50\% & 26.9 & 28.1 & 17.66 & 37.51 & 58.78 & 32.07 \\
        Ours 75\% & 26.5 & 28.9 & 17.27 & 37.63 & 58.85 & 32.16 \\
        \bottomrule
    \end{tabular}
    \label{tab:patch}
\end{table}





% \begin{table}[t]
%     \centering
%     \scriptsize
%     % \setlength{\tabcolsep}{2.0pt} % Default value: 6pt
%     % \renewcommand{\arraystretch}{1} % Default value: 1
%     \caption{\textbf{Ablation of Patch}. Image Condensation}
%     \begin{tabular}{lc|cc|cc}
%         \toprule
%         \multirow{3}{*}{Methods} & \multirow{3}{*}{FLOPS\scriptsize{(1e15)}} & \multicolumn{2}{c|}{MSCOCO} & \multicolumn{2}{c}{Flickr} \\
%         ~ & ~ & I2T & T2I & I2T & T2I \\
%         \toprule
%         Rand & 0 & 23.1 & 23.4 & 38.5 & 40.2 \\
%         \midrule
%         BTS & 6.60 & 26.5 & 27.8 & 41.2 & 41.4 \\
%         \midrule
%         Ours 25\% & 0 & 17.9 & 18.1 & 29.9 & 30.2  \\
%         Ours 25\% & 0 & 24.0 & 24.9 & 41.1 & 41.8 \\
%         Ours 50\% & 0 & 26.9 & 28.1 & 47.7 & 47.7 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:patch}
% \end{table}




==> content/tab/ablation/thresh.tex <==
% 测一下 cos sim, 观察随着 thresh 提升的=导致的 sim 是否有升高
\begin{table}[t]
    \centering
    \footnotesize
    \caption{\textbf{Ablation of Caption Enhancement}. Caption enhancement rely on classes from $\governorTXT$. We switch the threshold of class prediction confidence, and determine the captions to be enhanced.}
    % \vspace{-0.3cm}
    \begin{tabular}{lc|cc|cc}
        \toprule
        \multirow{2}{*}{Methods} & 
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Sample\\ (\%)\end{tabular}}
        & \multicolumn{2}{c|}{MSCOCO} & \multicolumn{2}{c}{Flickr} \\
        ~ & ~ & I2T & T2I & I2T & T2I \\
        \hline \hline
        Rand & 0 & 23.1 & 23.4 & 38.5 & 40.2 \\
        \midrule
        BTS & 0 & 26.5 & 27.8 & 41.2 & 41.4 \\
        \midrule
        1.0 & 0 & 26.4 & 27.4 & 47.1 & 46.6 \\
        0.3 & 43 & 26.2 & 27.4 & 47.3 & 47.6 \\
        0.5 & 35 & 26.9 & 28.1 & 47.7 & 47.7 \\
        0.7 & 21 & 26.5 & 28.0 & 47.6 & 47.0 \\
        \bottomrule
    \end{tabular}
    \label{tab:thresh}
\end{table}




==> content/tab/across_data.tex <==


\begin{table*}[htpb]
    \caption{\textbf{Comparison with different source of data.} the \gc{baseline}
    \begin{CJK*}{UTF8}{gbsn}\weixiong{表有点丑, 想表达 Juicer 对于不同 data 的通用性 1. 减少一些 benchmark 2. 减少对比的方法, 或者干脆用一个柱状图来表示结果?}\end{CJK*}
    }
    \label{tab:across_data}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{4.6pt} % Default value: 6pt
    \begin{tabular}{ll|cccccccccc}
        Dataset & Method & MSCOCO & Flickr & ImgN-R & ImgN-A & OKVQA & CCBench & HalBench & MMBench & MNMU & MMStar \\
        \shline
        \parbox[t]{4mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{CC3M}}} & \gc{Whole Dataset} & 5.8\blue{1.0} & 17.2\blue{1.0} & 24.4\blue{1.0} & 11.5\blue{1.0} & 30.1\blue{1.0} & 41.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} \\
        ~ & TLDR & 8.3 & 22.0 & 31.6 & 22.2 & 46.7  \\
        ~ & BNSL & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        ~ & SemDeDup & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        \arrayrulecolor{lightgray}\cline{2-12}\arrayrulecolor{black}
        \parbox[t]{4mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{CC12M}}} & \gc{Whole Dataset} & 5.8\blue{1.0} & 17.2\blue{1.0} & 24.4\blue{1.0} & 11.5\blue{1.0} & 30.1\blue{1.0} & 41.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} \\
        ~ & TLDR & 8.3 & 22.0 & 31.6 & 22.2 & 46.7  \\
        ~ & BNSL & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        ~ & SemDeDup & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        \hline
        \parbox[t]{4mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{YFCC}}} & \gc{Whole Dataset} & 5.8\blue{1.0} & 17.2\blue{1.0} & 24.4\blue{1.0} & 11.5\blue{1.0} & 30.1\blue{1.0} & 41.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} \\
        ~ & TLDR & 8.3 & 22.0 & 31.6 & 22.2 & 46.7  \\
        ~ & BNSL & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        ~ & SemDeDup & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        \arrayrulecolor{lightgray}\cline{2-12}\arrayrulecolor{black}
        \parbox[t]{4mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LAION}}} & \gc{Whole Dataset} & 5.8\blue{1.0} & 17.2\blue{1.0} & 24.4\blue{1.0} & 11.5\blue{1.0} & 30.1\blue{1.0} & 41.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} & 5.8\blue{1.0} \\
        ~ & TLDR & 8.3 & 22.0 & 31.6 & 22.2 & 46.7  \\
        ~ & BNSL & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
        ~ & SemDeDup & 10.2 & 26.7 & 36.5 & 10.3 & 25.3  \\
    \end{tabular}
\end{table*}




==> content/tab/all.tex <==

\begin{table*}[htpb]
    \centering
    \scriptsize
    % \renewcommand{\arraystretch}{1} % Default value: 1
    \caption{Raw Result. }
    % \vspace{-5pt}
    \begin{tabular}{lc|cccccc|cccccc|cccccc}
        \toprule
        \multirow{3}{*}{Methods} & \multirow{3}{*}{\#Samples} & \multicolumn{6}{c|}{MSCOCO} & \multicolumn{6}{c|}{Flickr} & \multicolumn{6}{c}{ImNet} \\
        ~ & ~ & ~ & I2T & ~ & ~ & T2I & ~ & ~ & I2T & ~ & ~ & T2I & ~ & \multicolumn{2}{c}{R} & \multicolumn{2}{c}{A} & \multicolumn{2}{c}{K} \\
        ~ & ~ & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 \\
        \toprule
        % \multirow{2}{*}{CLIP ~\cite{radford2021learning}} & CC3M & 2.82M & 11.0 & 31.0 & 43.0 & 9.0 & 28.0 & 41.0 \\
        % ~ & PAH100 & ~ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
        CLIP & 12m & 25.2 & 49.4 & 61.9 & 25.3 & 50.0 & 61.7 & 56.9 & 81.6 & 87.4 & 55.2 & 81.9 & 87.6 & 49.21 & 74.09 & 10.13 & 33.21 & 39.00 & 66.93 \\
        rand & 0.58M & 2.7 & 9.4 & 15.3 & 3.0 & 10.1 & 15.4 & 6.7 & 19.0 & 26.6 & 7.9 & 17.8 & 26.3 & 6.06 & 16.67 & 1.91 & 7.85 & 5.86 & 15.33 \\
        rand & 1.17M & 5.2 & 14.9 & 23.1 & 5.9 & 16.3 & 23.4 & 12.9 & 29.0 & 38.5 & 10.9 & 29.3 & 40.2 & 10.25 & 23.63 & 2.39 & 10.12 & 10.08 & 22.68 \\
        \midrule
        bts-500k-e50 & 0.58M & 2.9 & 10.3 & 15.6 & 3.4 & 10.8 & 17.2 & 6.7 & 18.7 & 26.6 & 7.1 & 18.7 & 26.6 & 7.42 & 18.71 & 1.80 & 6.67 & 5.89 & 14.23 \\
        bts-1m-e5 & 0.58M & 4.1 & 12.4 & 18.4 & 4.5 & 13.0 & 19.5 & 10.8 & 25.6 & 34.2 & 10.2 & 25.4 & 34.6 & 8.49 & 21.53 & 1.81 & 8.08 & 7.30 & 17.16 \\
        bts-1m-e15 & 0.58M & 3.6 & 11.7 & 18.1 & 4.4 & 12.8 & 18.9 & 8.9 & 23.2 & 32.1 & 8.7 & 23.7 & 31.9 & 8.40 & 20.77 & 1.68 & 7.31 & 7.01 & 16.71 \\
        bts-1m-e25 & 0.58M & 4.0 & 11.7 & 18.1 & 4.1 & 13.0 & 19.3 & 9.3 & 23.3 & 32.9 & 10.2 & 22.1 & 31.5 & 8.12 & 20.45 & 1.68 & 7.57 & 6.91 & 16.63 \\
        bts-500k-e6 & 1.17M &  \\
        bts-500k-e12 & 1.17M &  \\
        bts-500k-e25 & 1.17M &  \\
        bts-500k-e50 & 1.17M & 5.5 & 15.8 & 23.7 & 5.8 & 17.2 & 24.4 & 11.5 & 30.1 & 41.8 & 12.3 & 30.4 & 40.5 & 10.17 & 23.65 & 2.08 & 9.64 & 9.86 & 22.06 \\
        bts-1m-e50 & 1.17M & 6.1 & 18.9 & 27.2 & 6.5 & 19.4 & 28.0 & 14.4 & 31.2 & 41.5 & 13.2 & 31.1 & 41.5 & 12.13 & 26.55 & 2.48 & 9.64 & 10.65 & 23.62 \\
        bts-1m-e50(eval on e45) & 1.17M & 5.9 & 18.6 & 26.5 & 6.3 & 19.4 & 27.8 & 14.6 & 31.0 & 41.2 & 13.1 & 31.4 & 41.4 & 11.90 & 26.11 & 2.47 & 9.41 & 10.56 & 23.27 \\
        \midrule
        seed-p1 & 0.58M & 3.0 & 9.8 & 15.3 & 3.2 & 10.6 & 15.6 & 7.1 & 20.2 & 26.6 & 7.8 & 18.7 & 26.3 & 6.58 & 17.31 & 1.67 & 6.72 & 5.57 & 13.59 \\
        seed-p1 & 1.17M & 5.7 & 16.8 & 24.2 & 6.0 & 17.4 & 24.7 & 13.0 & 32.2 & 41.1 & 13.1 & 30.0 & 38.6 & 9.96 & 23.03 & 2.43 & 9.47 & 9.32 & 21.11 \\
        seed-p2 & 0.58M & 2.9 & 10.6 & 16.0 & 3.4 & 11.3 & 17.3 & 7.1 & 20.3 & 27.9 & 7.40 & 20.6 & 28.4 & 8.39 & 20.78 & 1.77 & 7.09 & 6.40 & 15.31 \\
        seed-p2 & 1.17M & 5.9 & 16.8 & 24.4 & 6.1 & 17.4 & 24.9 & 13.6 & 32.2 & 41.6 & 13.2 & 31.7 & 41.3 & 11.82 & 26.60 & 2.20 & 9.87 & 10.34 & 22.56 \\
        \midrule
        plip & 1M & 4.0 & 12.0 & 18.2 & 4.26 & 13.2 & 19.3 & 10.0 & 24.1 & 33.6 & 9.2 & 23.6 & 32.0 & 7.89 & 20.14 & 2.24 & 8.63 & 7.55 & 18.03 \\
        plip & 2M & 6.6 & 18.4 & 27.4 & 7.1 & 19.7 & 28.4 & 15.6 & 35.2 & 47.1 & 14.8 & 35.4 & 46.6 & 11.63 & 27.06 & 2.71 & 11.09 & 11.52 & 25.28  \\
        \bottomrule
    \end{tabular}
    \label{tab:raw-result}
\end{table*}





==> content/tab/classification.tex <==

\begin{table*}[htpb]
    \centering
    \footnotesize
    \caption{\textbf{Zero-shot Image Classification}. Our framework outperforms the BTS framework in a large margin.}
    \vspace{-0.2cm}
    \begin{tabular}{lccccc|cccccc}
        \toprule
        % \multirow{3}{*}{Method} & \multirow{3}{*}{Arch} & \multicolumn{2}{c}{\multirow{3}{*}{FLOPS\scriptsize{(1e17)}}} & \multicolumn{2}{c|}{\multirow{3}{*}{\#Samples(M)}} & \multicolumn{6}{c|}{MSCOCO} & \multicolumn{6}{c}{Flickr} \\
        % ~ & ~ & ~ & ~ & ~ & ~ & ~ & I2T & ~ & ~ & T2I & ~ & ~ & I2T & ~ & ~ & T2I & ~ \\
        % ~ & ~ & \scriptsize{Train} & \scriptsize{Pre} & \scriptsize {Seed} & \scriptsize{Train} & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
        \multirow{2}{*}{Methods} & \multirow{2}{*}{Arch} & \multicolumn{2}{c}{FLOPS\scriptsize{(1e17)}} & \multicolumn{2}{c|}{\#Samples(M)} & \multicolumn{2}{c}{ImgNet-R} & \multicolumn{2}{c}{ImgNet-A} & \multicolumn{2}{c}{ImgNet-K} \\
        ~ & ~ & Train & Pre & Seed & Train & Top1 & Top5 & Top1 & Top5 & Top1 & Top5 \\
        \hline \hline
        Rand & CLIP~\cite{radford2021learning} & 3.8 & 0 & 1 & 2 & 10.25 & 23.63 & 2.39 & 10.12 & 10.08 & 22.68 \\
        \midrule
        \multirow{6}{*}{BTS\cite{cheng2024visionlanguagemodelsselfimprovereasoning}} & \multirow{6}{*}{CLIP~\cite{radford2021learning}} & 4.3 & 0.6 & 1 & 2 & 10.17 & 23.65 & 2.08 & 9.64 & 9.86 & 22.06 \\
        ~ & ~ & 4.3 & 1.1 & 1 & 2 & 12.13 & 26.55 & 2.48 & 9.64 & 10.65 & 23.62 \\
        ~ & ~ & 4.3 & 2.2 & 1 & 2 & 11.90 & 26.11 & 2.47 & 9.41 & 10.56 & 23.27 \\
        ~ & ~ & 6.5 & 0.8 & 1 & 3 & 16.72 & 33.27 & 4.00 & 14.48 & 17.32 & 35.75 \\
        ~ & ~ & 6.5 & 1.6 & 1 & 3 & 18.15 & 35.28 & 4.56 & 16.63 & 19.69 & 39.57 \\
        ~ & ~ & 6.5 & 3.2 & 1 & 3 & 17.67 & 34.66 & 4.23 & 16.04 & 18.70 & 38.38 \\
        \midrule
        Ours\_v & \multirow{4}{*}{CLIP~\cite{radford2021learning}} & 2.5 & 0 & 0 & 2 & 11.63 & 27.06 & 2.71 & 11.09 & 11.52 & 25.28 \\
        Ours\_t & ~ & 2.5 & 0 & 0 & 2 & 12.34 & 29.46 & 2.55 & 11.51 & 15.17 & 33.42 \\
        Ours & ~ & 2.5 & 0 & 0 & 2 & 14.02 & 32.18 & 3.19 & 12.49 & 17.66 & 37.51 \\
        Ours & ~ & 3.8 & 0 & 0 & 3 & 25.01 & 48.31 & 4.37 & 16.29 & 20.61 & 42.38 \\
        \bottomrule
    \end{tabular}
    \label{tab:Zeroshot-Classification}
\end{table*}


==> content/tab/gen.tex <==
% 生成任务结果, 包括 captioning, vqa



\begin{table*}[htpb]
    \centering
    \scriptsize
    \caption{\textbf{All-Round Embedding Quality under For VLMs}. We train LLaVA1.5-13B by initializing its vision backbone with our image encoder, and the good results show better visual modeling for multi-modal foundation models.}
    % \vspace{-0.3cm}
    \begin{tabular}{lc|ccccccccccc}
        \toprule
        Methods & 
        \begin{tabular}[c]{@{}c@{}}FLOPS\\ \scriptsize{(1e15)}\end{tabular}
        & OKVQA & CCBench & HalBench & MMBench & MNMU & MMStar & OCRVQA & POPE & SciQA & SEEDBench & TextVQA \\
        % ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\
        \hline \hline
        Rand & 0 & 34.24 & 1.57 & 29.12 & 15.72 & 24.33 & 14.73 & 2.80 & 65.15 & 44.52 & 18.39 & 1.31 \\
        \midrule
        BTS & 3.30 & 48.68 & 1.09 & 28.30 & 24.13 & 22.81 & 26.03 & 11.07 & 62.21 & 60.07 & 34.28 & 1.51 \\
        BTS & 6.60 & 50.48 & 1.17 & 27.76 & 24.31 & 26.11 & 20.53 & 12.37 & 62.35 & 61.18 & 34.21 & 1.73 \\
        \midrule
        Ours & 0 & 58.78 & 1.18 & 32.07 & 38.32 & 32.67 & 24.73 & 24.51 & 71.77 & 63.66 & 42.34 & 3.23 \\
        \bottomrule
    \end{tabular}
    \label{tab:Gen}
\end{table*}

